Towards a Skill- And Ability-Based Development Process for Self-Aware Automated Road Vehicles

The development of fully automated vehicles imposes new challenges in the development process and during the operation of such vehicles. As traditional design methods are not sufficient to account for the huge variety of scenarios which will be encountered by (fully) automated vehicles, approaches for designing safe systems must be extended in order to allow for an ISO~26262 compliant development process. During operation of vehicles implementing SAE Levels 3+ safe behavior must always be guaranteed, as the human driver is not or not immediately available as a fall-back. Thus, the vehicle must be aware of its current performance and remaining abilities at all times. In this paper we combine insights from two research projects for showing how a skill- and ability-based approach can provide a basis for the development phase and operation of self-aware automated road vehicles.

==> bilder/shapes.tex <==
%
% declare a new shape for the service interface
\makeatletter
\pgfdeclareshape{openinterface}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
}
\pgfdeclareshape{interface}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{.95\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
  \foregroundpath{
	 \centerpoint
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
    \pgfutil@tempdimb=\radius%      \pgfutil@tempdima = radius
	 \advance\pgfutil@tempdima by-.25\pgfutil@tempdima%
	 \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+.25\pgfutil@tempdimb}{0pt}}}{\pgfutil@tempdima}
	 \pgfusepath{fill}
  }
}
% UML component
\pgfdeclareshape{umlcomponent}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \backgroundpath{
	  \newdimen\pgf@xd\newdimen\pgf@yd
	  \newdimen\pgf@xe\newdimen\pgf@ye
	  \newdimen\pgf@xf\newdimen\pgf@yf
		% store lower right in xa/ya and upper right in xb/yb
		\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		% compute west point as well as vertical distance and height of decoration
		\pgf@xc=\pgf@xa \pgf@yc=.5\pgf@yb \advance\pgf@yc by .5\pgf@ya
		\pgf@yd=.3\pgf@yb
		\pgf@ye=.2\pgf@yb
%		% compute position of second decoration in xe/ye and xf/yf
%		\pgf@xe=\pgf@xa \pgf@ye=.1\pgf@y
%		\pgf@xf=\pgf@xa \pgf@yf=.2\pgf@ya
		% draw main shape
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathclose
		% draw internal lines
		\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd}}
  }
}

% arrows
\pgfarrowsdeclare{srvarrow}{srvarrow}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{0.4\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.5\pgfutil@tempdima}{0.94\pgfutil@tempdima}}}%
  \pgfpatharc{110}{-110}{\pgfutil@tempdima}
  \pgfsetfillcolor{white}
  \pgfusepathqfill
  \pgftransformshift{\pgfqpoint{0.35\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.8\pgfutil@tempdima}{0.94\pgfutil@tempdima}}}%
  \pgfpatharc{110}{-110}{\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqstroke
  \pgftransformshift{\pgfqpoint{-0.5\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.55\pgfutil@tempdima}{.98\pgfutil@tempdima}}}%
  \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+0.2\pgfutil@tempdimb}{0pt}}}{0.75\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqfill
}

\pgfarrowsdeclare{srvrequired}{srvrequired}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{0.35\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{1.3\pgfutil@tempdima}{0.95\pgfutil@tempdima}}}%
  \pgfpatharc{80}{280}{\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqstroke 
}

\pgfarrowsdeclare{srvprovided}{srvprovided}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.4\pgfutil@tempdima}{.98\pgfutil@tempdima}}}%
  \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+0.2\pgfutil@tempdimb}{0pt}}}{0.75\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqfill 
}
\makeatother

